The Arabic Parallel Gender Corpus 2.0: Extensions and Analyses

Gender bias in natural language processing (NLP) applications, particularly machine translation, has been receiving increasing attention. Much of the research on this issue has focused on mitigating gender bias in English NLP models and systems. Addressing the problem in poorly resourced, and/or morphologically rich languages has lagged behind, largely due to the lack of datasets and resources. In this paper, we introduce a new corpus for gender identification and rewriting in contexts involving one or two target users (I and/or You) -- first and second grammatical persons with independent grammatical gender preferences. We focus on Arabic, a gender-marking morphologically rich language. The corpus has multiple parallel components: four combinations of 1st and 2nd person in feminine and masculine grammatical genders, as well as English, and English to Arabic machine translation output. This corpus expands on Habash et al. (2019)'s Arabic Parallel Gender Corpus (APGC v1.0) by adding second person targets as well as increasing the total number of sentences over 6.5 times, reaching over 590K words. Our new dataset will aid the research and development of gender identification, controlled text generation, and post-editing rewrite systems that could be used to personalize NLP applications and provide users with the correct outputs based on their grammatical gender preferences. We make the Arabic Parallel Gender Corpus (APGC v2.0) publicly available.

==> table2.tex <==
\begin{table*}[h]
\begin{center}
\setlength{\tabcolsep}{2pt}
\scalebox{0.80}{
\begin{tabular}{|l|r|c|c|r|c}
\cline{1-5}

\multicolumn{1}{|c|}{\bf English} & \multicolumn{1}{c|}{\bf Arabic} & \bf Label & \bf Reinflection Label & \multicolumn{1}{c|}{\bf Reinflection} \\\cline{1-5}\cline{1-5}




 &  & & FM & \textcolor{red}{\<ترحل>} \<يجب أن> \textcolor{blue}{\<آسفة>} & (k) \\
I'm \textcolor{blue}{sorry}, you're going to have to \textcolor{red}{leave} & \textcolor{red}{\<ترحل>} \<يجب أن> \textcolor{blue}{\<آسف>} & MM & MF & \textcolor{red}{\<ترحلي>} \<يجب أن> \textcolor{blue}{\<آسف>} & (l) \\
 & & & FF & \textcolor{red}{\<ترحلي>} \<يجب أن> \textcolor{blue}{\<آسفة>} & (m) \\\cline{1-5}

 & &  & MM & \textcolor{red}{\<عزيزي>}  \<للغاية يا>  \textcolor{blue}{\<خائف>}  \<أنا> & (n) \\
 \textcolor{red}{Baby}, I'm so \textcolor{blue}{scared} right now & \textcolor{red}{\<عزيزي>}  \<للغاية يا>  \textcolor{blue}{\<خائفة>} \<أنا> & FM & FF & \textcolor{red}{\<عزيزتي>}  \<للغاية يا>  \textcolor{blue}{\<خائفة>}  \<أنا> & (o) \\
 & & & MF & \textcolor{red}{\<عزيزتي>}  \<للغاية يا>  \textcolor{blue}{\<خائف>}  \<أنا> & (p) \\\cline{1-5}
 
  &  &  & FF & \textcolor{red}{\<أماه>} \<بعودتك يا> \textcolor{blue}{\<سعيدة>} \<أنا> & (q) \\
I'm \textcolor{blue}{glad} you made it home, \textcolor{red}{mom}  & \textcolor{red}{\<أماه>} \<بعودتك يا> \textcolor{blue}{\<سعيد>} \<أنا> & MF & MM & \textcolor{red}{\<أبتاه>}  \<بعودتك يا> \textcolor{blue}{\<سعيد>} \<أنا> & (r) \\
 & & & FM & \textcolor{red}{\<أبتاه>}  \<بعودتك يا> \textcolor{blue}{\<سعيدة>} \<أنا> & (s) \\\cline{1-5}
 
  & & & MF & \textcolor{blue}{\<بالغبي>} \textcolor{red}{\<تناديني>} \<لا> & (t) \\
 Don't \textcolor{red}{call} me a \textcolor{blue}{fool} & \textcolor{blue}{\<بالغبية>} \textcolor{red}{\<تناديني>} \<لا> & FF & FM & \textcolor{blue}{\<بالغبية>} \textcolor{red}{\<تنادني>} \<لا> & (u) \\
 & & & MM & \textcolor{blue}{\<بالغبي>} \textcolor{red}{\<تنادني>} \<لا> & (v) 
 \\\cline{1-5}
 
 

\end{tabular}
}
\end{center}
\caption{}
% \caption{Examples from the Arabic Parallel Gender Corpus including original sentence, its gender and its reinflection to the opposite gender where appropriate.}
\label{tab:first-and-second-example}
\end{table*}

==> table3_word_level_examples_old.tex <==
\begin{table*}[h]
\begin{center}
\setlength{\tabcolsep}{2pt}
\scalebox{0.85}{
\begin{tabular}{|l|r|c|c|r|c}
\cline{1-5}

\multicolumn{1}{|c|}{\bf English} & \multicolumn{1}{c|}{\bf Arabic} & \bf Label & \bf Reinflection Label & \multicolumn{1}{c|}{\bf Reinflection} & \\\cline{1-5}


I wanna thank you & \<أريد أن أشكرك> & BB &  & & (a)\\
 & B~~~~~B~~~~~~B &  &  & & \\\cline{1-5}
I have something to say & \<لدي شيء لأقوله> & BN &  &  & (b)\\
 & B~~~~~B~~~~~~B &  &  & & \\\cline{1-5}
I'm so  \textcolor{blue}{happy} for you & \<من أجلك> \textcolor{blue}{\<سعيدة>} \<أنا> & FB & MB & \<من أجلك> \textcolor{blue}{\<سعيد>} \<أنا> & (c)\\
& B~~~~~B~~~~\textcolor{blue}{1F}~~~~~B &  &  & B~~~B~~~\textcolor{blue}{1M}~~~~B & \\\cline{1-5}

We were  \textcolor{blue}{coming} to see you & \<لرؤيتك> \textcolor{blue}{\<قادمات>} \<نحن> & F!B & M!B & \<لرؤيتك> \textcolor{blue}{\<قادمون>} \<نحن> & (d) \\

&  B~~~~~~~\textcolor{blue}{1F!}~~~~~B & &  & B~~~~~~\textcolor{blue}{1M!}~~~~~B  & \\\cline{1-5}
% Because I'm your big \textcolor{blue}{brother}  &\<الكبير>  \textcolor{blue}{ \<أخوك> } \<لأنني>  & MB & FB & \<الكبيرة> \textcolor{blue}{\<أختك>}  \<لأنني> & (e) \\\cline{1-5}
% We're \textcolor{blue}{ready}  & \textcolor{blue}{\<مستعدون>} \<نحن> & M!B & F!B & \textcolor{blue}{\<مستعدات>} \<نحن> & (f) \\\cline{1-5}\cline{1-5}
I know, \textcolor{red}{babe}  & \textcolor{red}{\<عزيزتي>} \<أعلم ذلك يا> & BF & BM &  \textcolor{red}{\<عزيزي>} \<أعلم ذلك يا> & (e)\\
& \textcolor{red}{2F}~~~~~B~~~~B~~~~~B &  &  & \textcolor{red}{2M}~~~~~B~~~~B~~~~~B  & \\\cline{1-5}
I \textcolor{red}{respect} you [pl]  &   \textcolor{red}{\<أحترمكن>}   \<أنا> & BF! & BM! &  \textcolor{red}{\<أحترمكم>} \<أنا> & (f)\\
&   \textcolor{red}{2F!}~~~~B & &  &  \textcolor{red}{2M!}~~~~B & \\\cline{1-5}
% I'm right here \textcolor{red}{dad}  & \textcolor{red}{\<أبي>}  \<أنا هنا يا> & BM & BF & \textcolor{red}{\<أمي>} \<أنا هنا يا> & (i) \\\cline{1-5}
% I \textcolor{red}{love} you [pl] so much  & \<كثيرا> \textcolor{red}{\<أحبكم>} & BM! & BF! &  \<كثيرا> \textcolor{red}{\<أحبكن>} & (j) \\\cline{1-5}\cline{1-5}

 & &  & MM & \textcolor{red}{\<عزيزي>}  \<للغاية يا>  \textcolor{blue}{\<خائف>}  \<أنا> & (g)\\
 & &  &  & \textcolor{red}{2M}~~~~B~~~~B~~~~\textcolor{blue}{1M}~~~~~B  & \\
 \textcolor{red}{Baby}, I'm so \textcolor{blue}{scared} right now & \textcolor{red}{\<عزيزي>}  \<للغاية يا>  \textcolor{blue}{\<خائفة>} \<أنا> & FM & FF 
 & \textcolor{red}{\<عزيزتي>}  \<للغاية يا>  \textcolor{blue}{\<خائفة>}  \<أنا> & (h)\\
 & \textcolor{red}{2M}~~~~B~~~~B~~~~\textcolor{blue}{1F}~~~~~B   &  &  & \textcolor{red}{2F}~~~~B~~~~B~~~~\textcolor{blue}{1F}~~~~~B   & \\
 & & & MF & \textcolor{red}{\<عزيزتي>}  \<للغاية يا>  \textcolor{blue}{\<خائف>}  \<أنا> & (i)\\
 & &  &  & \textcolor{red}{2F}~~~~B~~~~B~~~~\textcolor{blue}{1M}~~~~~B  & \\\cline{1-5}

 
\end{tabular}
}
\end{center}
\caption{Examples of word-level gender annotation. First person gendered words are in \textcolor{blue}{blue} and second person gendered words are in \textcolor{red}{red}.}
\label{tab:word-level-example}
\end{table*}

==> table9_EN_examples.tex <==
\begin{table}
    \parbox{\columnwidth}{
    \centering
        \begin{tabular}{|c|c|}
        \hline
        \bf English Noun & \bf Gender \\\hline
        Teacher & B \\\hline
        Scientist  & B \\\hline
        Prostitute & B \\\hline\hline
        Father & M \\\hline
        Policeman & M \\\hline
        Actor & M\\\hline\hline
        Mother & F \\\hline
        Queen & F \\\hline
        Waitress & F\\\hline
        \end{tabular}
    \caption{Examples of gender specific English nouns in our corpus.}
    \label{tab:en-nouns}
    }
\end{table}

==> testing_table.tex <==
% \begin{table*}[t!]
% \begin{center}
% \scalebox{0.78}{

% \begin{tabular}{|r|r|r||c|c|  c  |c|c|c||r|}
% \cline{4-5}\cline{7-9}
% \multicolumn{3}{c|}{}  & \multicolumn{1}{c|}{\bf Original Corpus} &   & \multicolumn{3}{c|}{\bf Balanced Corpus} & \multicolumn{1}{c}{}  \\\cline{4-5}\cline{7-9}

% \multicolumn{3}{c}{}  & \multicolumn{1}{c}{(a)}             & \multicolumn{1}{c|}{}      & & \multicolumn{1}{c}{(c)}   & \multicolumn{1}{c}{(d)}       & \multicolumn{1}{c}{(e)}     &  \multicolumn{1}{c}{}   \\\cline{1-4}\cline{7-10}
% \bf Sentences         &\bf  Words & \bf   Words$^{MF}$     &  \bf Input  &   & &  \bf Input & \bf Target$^M$ &  \bf Target$^F$ & \bf Sentences  \\\cline{1-4}\cline{7-10}
% 10,242            & 74,702     & 0              & B               &            & & B     & B        & B        & 10,242    & 74,702     & 0              \\\cline{1-5}\cline{7-12}
%  362              & 2,720      & 422            & F               & M$^r$    &  & F     & M$^r$       & F        & 362      & 2,720      & 422            \\\cline{1-5}\cline{7-12}
%  636              & 4,710      & 743            & M               & F$^r$      &    & M     & M        & F$^r$       & 636      & 4,710      & 743            \\\cline{1-5}\cline{7-12}
%  \multicolumn{6}{c|}{} &  M$^r$    & M$^r$       & F        & 362      & 2720      & 422            \\\cline{7-12}
%   \multicolumn{6}{c|}{}      & F$^r$   & M        & F$^r$       & 636      & 4,710      & 743           \\\cline{1-3}\cline{1-3}\cline{7-12}\cline{7-12}
%  11,240            & 82,132     & \multicolumn{1}{c|}{1,165 }          &    \multicolumn{6}{c|}{}       & 12,238    & 89,562     & 2,330  \\\cline{1-3}\cline{10-12}          
% \end{tabular}
% }
% \end{center}
% \caption{Statistics of the original corpus we annotated and the balanced version we report on in the paper experiments. Words$^{MF}$ refers to the count of gender-marking words, specifically. M$^r$   and F$^r$ are the reinflected versions of the F and M labelled sentences, respectively, in the same rows they appear in.  }
% \label{tab:corpus-stats}
% \end{table*}

==> testing_table2.tex <==
% \begin{table*}
%     \parbox{.4\linewidth}{
%     \centering
%     \scalebox{0.8}{
%         \begin{tabular}{|r|c|ccc|}
%             \cline{2-5}
%             \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{\bf Original Corpus}\\\cline{1-5}
%             \bf Sentences &\bf  Label &  \multicolumn{3}{c|}{\bf Reinflection Label}\\\cline{1-5}
%             36,980 & BB &  & & \\\hline\hline
%             5,208  & BF &  & BM & \\\cline{1-5}
%             12,166  & BM &   & BF & \\\hline\hline
%             1,123   & FB &  & FM &  \\\cline{1-5}
%             1,940   & MB &  & FB &   \\\hline\hline
%             68   & FF &  MF & FM & MM  \\\cline{1-5}
%             135   & FM &  MM & FF & MF  \\\cline{1-5}
%             117   & MF &  FF & MM & FM   \\\cline{1-5}
%             298   & MM &  FM & MF & FF  \\\cline{1-5}
%             58,035   & \multicolumn{4}{c}{}  \\\cline{1-1}
%         \end{tabular}
        
%     }
%     \caption{Sentence-level statistics of the \\ original corpus. }
%     \label{tab:sentence-level-stats-orig}
%     }
%     \quad
%     \parbox{.5\linewidth}{
%     \centering
%     \scalebox{0.8}{
%         \begin{tabular}{|c|c|c|c|c|r|}
%             \cline{1-5}
%             \multicolumn{5}{|c|}{\bf Balanced Corpus}\\\cline{1-6}
            
%             \bf Input & \bf Target\textsubscript{\textit{MM}} &  \bf Target\textsubscript{\textit{FM}} & \bf Target\textsubscript{\textit{MF}} &  \bf Target\textsubscript{\textit{FF}} &  \bf Sentences  \\\cline{1-6}
            
%             BB & BB &  BB  & BB  &  BB &  36,980 \\\hline\hline
            
%             BF & BM &  BM  & BF &  BF & 17,374 \\\cline{1-6}
            
%             BM & BM & BM & BF & BF  &  17,374 \\\hline\hline
            
%             FB & MB &  FB & MB &  FB &  3,063 \\\cline{1-6}
            
%             MB & MB &  FB  & MB &  FB & 3,063  \\\hline\hline
            
%             FF & MM &  FM & MF &  FF & 618  \\\cline{1-6}
            
%             FM & MM &  FM & MF &  FF & 618  \\\cline{1-6}
            
%             MF & MM & FM & MF & FF & 618  \\\cline{1-6}
            
%             MM & MM & FM & MF & FF  & 618  \\\cline{1-6}
            
%             \multicolumn{5}{c|}{}   & 80,326  \\\cline{6-6}
            
%             \end{tabular}
%         }
%     \caption{Sentence-level statistics of the balanced corpus and its five versions.}
%     \label{tab:sentence-level-stats-balanced}
%     }
% \end{table*}



% \begin{table*}[t!]
% \begin{center}
% \scalebox{0.75}{

% \begin{tabular}{|r|c|ccc|  ccc  |c|c|c|c|c|r|}
% \cline{2-5}\cline{9-13}
% \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{\bf Original Corpus} & & & & \multicolumn{5}{c|}{\bf Balanced Corpus} & \multicolumn{1}{c}{} \\\cline{1-5}\cline{9-14}

% \bf Sentences &\bf  Sentence Tag &  \multicolumn{3}{|c|}{\bf Manual Reinflection}   &  & & &  \bf Input & \bf \bf Target\textsubscript{\textit{MM}} &  \bf Target\textsubscript{\textit{FM}} & \bf \bf Target\textsubscript{\textit{MF}} &  \bf \bf Target\textsubscript{\textit{FF}} & \bf Sentences  \\\cline{1-5}\cline{9-14}

% 36,980 & BB &  & & & & & & BB & BB & BB & BB &  BB & 36,980  \\\cline{1-5}\cline{9-14}

% 5,208  & BF &  & BM & &  & & & BF & BM &  BM  & BF &  BF & 17,374  \\\cline{1-5}\cline{9-14}

% 12,166  & BM &   & BF & & & & & BM & BM & BM & BF & BF  & 17,374 \\\cline{1-5}\cline{9-14}

% 1,123   & FB &  & FM & & & & & FB & MB &  FB & MB &  FB & 3,063  \\\cline{1-5}\cline{9-14}

% 1,940   & MB &  & FB & & & & & MB & MB &  FB  & MB &  FB  & 3,063   \\\cline{1-5}\cline{9-14}

% 68   & FF &  MF & FM & MM & & & & FF & MM &  FM & MF &  FF & 618  \\\cline{1-5}\cline{9-14}

% 135   & FM &  MM & FF & MF & & & & FM & MM &  FM & MF &  FF & 618  \\\cline{1-5}\cline{9-14}

% 117   & MF &  FF & MM & FM & & & & MF & MM & FM & MF & FF & 618   \\\cline{1-5}\cline{9-14}

% 298   & MM &  FM & MF & FF & & & & MM & MM & FM & MF & FF & 618   \\\cline{1-5}\cline{9-14}
% 58,035   & \multicolumn{4}{c}{} & & &   \multicolumn{6}{c|}{} & 80,326   \\\cline{1-1}\cline{14-14}

% \end{tabular}
% }
% \end{center}
% \caption{}
% \label{tab:corpus-stats}
% \end{table*}




==> testing_tableX.tex <==
% \begin{table*}[t!]
% \begin{center}
% \scalebox{0.75}{

% \begin{tabular}{|r|c|ccc|  ccc  |c|c|c|c|c|r|}
% \multicolumn{1}{c}{} & \multicolumn{4}{c}{\bf(a)} & & & \multicolumn{6}{c}{\bf (b)} & \multicolumn{1}{c}{} \\
% \cline{2-5}\cline{9-13}
% \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{\bf Original Corpus} & & & & \multicolumn{5}{c|}{\bf Balanced Corpus} & \multicolumn{1}{c}{} \\\cline{1-5}\cline{9-14}

% \bf Sentences &\bf  Sentence Tag &  \multicolumn{3}{c|}{\bf Manual Reinflection}   &  & & &  \bf Input & \bf \bf Target\textsubscript{\textit{MM}} &  \bf Target\textsubscript{\textit{FM}} & \bf \bf Target\textsubscript{\textit{MF}} &  \bf \bf Target\textsubscript{\textit{FF}} & \bf Sentences  \\\cline{1-5}\cline{9-14}

% 36,980 & BB &  & & & & & & BB & BB & BB & BB &  BB & 36,980  \\\hhline{*{5}{=}*{3}{~}*{6}{=}}
% 5,208  & BF &  & BM & &  & & & BF & BM &  BM  & BF &  BF & 17,374  \\\cline{1-5}\cline{9-14}

% 12,166  & BM &   & BF & & & & & BM & BM & BM & BF & BF  & 17,374 \\\hhline{*{5}{=}*{3}{~}*{6}{=}}

% 1,123   & FB &  & FM & & & & & FB & MB &  FB & MB &  FB & 3,063  \\\cline{1-5}\cline{9-14}

% 1,940   & MB &  & FB & & & & & MB & MB &  FB  & MB &  FB  & 3,063   \\\hhline{*{5}{=}*{3}{~}*{6}{=}}

% 68   & FF &  MF & FM & MM & & & & FF & MM &  FM & MF &  FF & 618  \\\cline{1-5}\cline{9-14}

% 135   & FM &  MM & FF & MF & & & & FM & MM &  FM & MF &  FF & 618  \\\cline{1-5}\cline{9-14}

% 117   & MF &  FF & MM & FM & & & & MF & MM & FM & MF & FF & 618   \\\cline{1-5}\cline{9-14}

% 298   & MM &  FM & MF & FF & & & & MM & MM & FM & MF & FF & 618   \\\cline{1-5}\cline{9-14}
% 58,035   & \multicolumn{4}{c}{} & & &   \multicolumn{6}{c|}{} & 80,326   \\\cline{1-1}\cline{14-14}

% \end{tabular}
% }
% \end{center}
% \caption{}
% \label{tab:corpus-stats}
% \end{table*}
